CrowdEst: A Method for Estimating (and not Simulating) Crowd Evacuation Parameters in Generic Environments

Evacuation plans have been historically used as a safety measure for the construction of buildings. The existing crowd simulators require fully-modeled 3D environments and enough time to prepare and simulate scenarios, where the distribution and behavior of the crowd needs to be controlled. In addition, its population, routes or even doors and passages may change, so the 3D model and configurations have to be updated accordingly. This is a time-consuming task that commonly has to be addressed within the crowd simulators. With that in mind, we present a novel approach to estimate the resulting data of a given evacuation scenario without actually simulating it. For such, we divide the environment into smaller modular rooms with different configurations, in a divide-and-conquer fashion. Next, we train an artificial neural network to estimate all required data regarding the evacuation of a single room. After collecting the estimated data from each room, we develop a heuristic capable of aggregating per-room information so the full environment can be properly evaluated. Our method presents an average error of 5% when compared to evacuation time in a real-life environment. Our crowd estimator approach has several advantages, such as not requiring to model the 3D environment, nor learning how to use and configure a crowd simulator, which means any user can easily use it. Furthermore, the computational time to estimate evacuation data (inference time) is virtually zero, which is much better even when compared to the best-case scenario in a real-time crowd simulator.

==> 1_intro.tex <==
\sloppy 

As new buildings are designed and constructed by engineers and architects, evacuation procedures to assure the needed safety standards are a major concern. Evacuation drills are usually used to analyze and evaluate predefined evacuation plans, but despite presenting strong similarities with real-world emergency scenarios \cite{pauls1980building}, they still pose significant ethical, practical, and financial challenges to be addressed \cite{gwynne1999review}. % TO DO: pegar mais descrição dessa referencia pra ficar bonitão

Crowd simulation is an interesting tool for evaluating real-world behavior of crowds in controlled scenarios. It can be defined as the process of simulating the movement of large amounts of agents, or crowds, in a previously-defined environment. The different ways in which crowds can behave has been object of research for almost thirty years \cite{survey2015}, including a variety of fields such as architecture, computer graphics, physics, robotics, safety engineering, training systems, psychology, and sociology \cite{survey2015,soraia2013crowd}.

%RCB: (1) evitar voz passiva; (2) Oxford comma nas enumerações, e.g.: this, that, <-- and also that.
% When simulating crowds, one should consider a set of parameters that coherently reproduce the desired scenario. Cassol et al.
% %SO: foi ele que definiu isso? Ele não citou de alguem? | EST: ta definido na introdução, na primeira pagina do artigo sem citar ninguém mesmo
% \cite{Cassol2017} categorized those parameters in the following taxonomy: 

% \begin{itemize}
% \item \textit{Physical Structure}: dimensions, number of floors, number of rooms, location of exits, and stairs; 
% \item \textit{Functionality}: whether people act as though they were in an office, hospital, school, airport, stadium, or arena; 
% \item \textit{Population}: number and spatial distribution of people in the environment, age, gender, relationships among them, knowledge about the environment; and 
% \item \textit{Event Conditions}: factors that may affect the navigability on the scenario, such as time (day or night), smoke, fire, or heat. 
% \end{itemize}

Regarding evacuation planning, crowd simulation can be used to evaluate evacuation plans, given a parametrized environment. For instance, Cassol et al. \cite{Cassol2017} employed \textit{CrowdSim}~\cite{Galea:1998,cassol:2016,Cassol:2012}, which is a crowd simulator tested and validated in real-world scenarios, to create and gather data from simulations. They also employed CMA-ES~\cite{hansen1996cma-es,hansen2011cma-es}, an evolutionary computation approach to vary the population data so that different portions of the crowd follow different routes. The simulation data was then evaluated using the $ep$ metric~\cite{cassol:2016} in order to find which route configuration was best-suited for evacuation (more details on the metric in~\cite{Cassol2017}). 

Albeit simple, when considering all  possible variations an environment can have, a very large quantity of simulations have to be executed, growing exponentially as more details are added to that environment. Even though simulations can run in a similar time needed for real-world evacuation drills, it is still the most computationally-demanding step in such an evacuation planning approach. 

\blue{Hence, this paper presents a method which goal is to estimate results of a certain evacuation scenario without the need of actually doing simulations in a complex environment during runtime. For achieving this goal, we divide the environment to be analyzed into a set of simplistic connected rooms. We hypothesize that by estimating the evacuation data on each room, we are capable of properly estimating the required information for the environment as a whole. For estimating per-room data, we make use of a machine learning approach, namely Artificial Neural Networks (ANN), which are previously trained on data collected from a number of simulation scenarios simulated beforehand. Furthermore, we defined a proper heuristic to unify per-room data in complex environments that comprise a set of connected rooms. To the best of our knowledge, this is the first work to makes use of a hybrid machine learning and crowd simulation approach for the task of evacuation planning in generic environments.}
%To the best of our knowledge, the objective of most works that uses machine learning in the crowds area is to count and estimate the quantity or density of peoples over an image of a crowd, only a few attempts were made to use machine learning together with crowd simulation for the task of evacuation planning.

%during environment parameters and the evacuation data from the rooms it connects. In order to coherently estimate evacuation data we investigated the usage of machine learning and neural networks algorithms using data generated in crowd simulator as the input. %validated with \textit{CrowdSim}. 
% This estimation of crowd evacuation scenarios using ANN is the main contribution of this work, since it is a new approach for Crowd Behavior as far as we know. We did not find any other work that used machine learning in crowd simulation area with similar purposes.

%------------------------------

This paper is organized as follows. Section~\ref{sec:related} presents related work on crowd simulation and evacuation planning. Section~\ref{sec:dev} describes our new approach for evacuation planning based on machine learning and crowd simulation. Section~\ref{sec:results} reports the results of a detailed experimental analysis for validating our new approach, whereas in Section~\ref{sec:remarks} we discuss our findings and point to future work directions.
%Finally, in Section~\ref{sec:remarks} we will provide insight about what still needs to be developed and how we plan to do it.

==> 2_related.tex <==
The study and modeling of crowd traffic and their behavior, as well as the environment and evacuation characteristics is vital to the use of critical spaces \cite{Fruin:1971,ma2014pedestrian,polus1983pedestrian,schadschneider2011empirical}. %Despite the fact that we have not found any approach that addresses  in the literature, 
Next, we briefly review some existing papers in areas related to our study: crowd simulation, evacuation planning, and crowd learning. We are not exhaustive in our analysis since the majority of them are not focused in the exact problem we address on this work.


\subsection{Crowd simulation}
Several studies were proposed to elaborate ways of simulating crowds in egress scenarios. Examples of crowd-simulation tools include the already-mentioned \textit{CrowdSim} \cite{Galea:1998,Cassol:2012,cassol:2016}, as well as SAFEgress~\cite{Chu:2014}, MIMOSA~\cite{Huangreal:2010}, and BioCrowds~\cite{Bicho:2009}.

\textit{SAFEgress} (Social Agent For Egress) \cite{Chu:2014} is a force-based approach that models evacuating pedestrians which are able to make their actions according to their knowledge of the environment and their interactions with the social groups and neighboring crowds.

MIMOSA: Mine Interior Model Of Smoke and Action \cite{Huangreal:2010} is a specific application of agent modeling within the context of a virtual underground coal mine, with a fire and smoke propagation model, and a human physiology and behavioral model.

\textit{BioCrowds} \cite{Bicho:2009} is a biologically-motivated approach that simulates crowds using a space-colonization algorithm, recreating several real crowds behaviors such as collision avoidance, speed reduction effect, and lane formation.

The work in \cite{Ji:2013,Aik:2012,Fu:2014} makes use of cellular automata to reproduce pedestrian behavior and exit selection using a least-effort cellular automaton algorithm, in which the motions and goals are probabilistic.

Van Den Berg et al. \cite{ORCA} proposed the method \textit{Optimal Reciprocal Collision Avoidance} ($ORCA$), used for robots to avoid collisions with each other. The method searches for the optimal velocity for each agent to move so all agents move through the environment without colliding. For that, it predicts the future positions of other agents and prioritizes velocities that minimize the probability of them colliding, ensuring that the agents adopt the velocities that will result in the lowest number of collisions by the time it performed the predictions.

\subsection{Evacuation planning}
Regarding evacuation planning, the work of Cassol et al. \cite{Cassol2017} makes use of crowd simulation (\textit{CrowdSim}) and evolutionary strategies (CMA-ES) to search for the best configuration of routes for evacuation within a given environment. 

Similarly, Garrett et al. \cite{garrett2006evacuation} employ Evolutionary Computation methods to evolve the placements of exits and other equipments in an effort to minimize the simulated evacuation time of the environment occupants. The simulation is made using an artificial potential-fields model in which exits attract agents and obstacles and other agents repel them.

\subsection{Crowd learning}
%In the crowd learning area we did not find works directly related to our work. Currently, a great focus of the area is on the crowd counting problem, also called density estimation. Chan et al. \cite{learning:chan2008privacy} created a privacy-preserving system for estimating the size of inhomogeneous crowds in a video, by segmenting it using a dynamic texture motion model, the correspondence of each segmented region's features and the number of people in it is estimated with a Gaussian Process regression. 
% by segmenting it using a dynamic texture motion model and extracting the features of each segmented region, the correspondence of the features and the number of people is estimated with a Gausean Process regression.

Currently the crowd learning area is heavily focusing on the crowd counting problem, also called density estimation. %Chan et al.~\cite{learning:chan2008privacy} create a privacy-preserving system for estimating the size of inhomogeneous crowds in a video, by segmenting it using a dynamic texture motion model and by analyzing the correspondence of features between each segmented region. The number of people in a video is finally estimated with Gaussian Process regression. %RCB: está bem estranha esta explicação do método
%EST: reescrevi abaixo mas acho que vou ler o artigo de novo pra redescrever melhor
Chan et al.~\cite{learning:chan2008privacy} created a privacy-preserving system for estimating the size of inhomogeneous crowds in a video. By segmenting the video and analyzing features detected between the frames and regions the number of people is estimated using Gaussian Process regression.
Similarly, Fradi et al.~\cite{learning:fradi2013crowd} extract features from videos and use a Gaussian symmetric kernel function to generate a crowd density map, allowing more specific locations of potentially crowded area. 

Liu et al. \cite{mubassir2017} is the closest approach to our work. They make use of artificial neural networks to learn the behavior of simulated crowds with the objective of replacing simulation with estimations, which is basically our same goal. They simulate the crowd on a fixed environment containing mobile parts whose disposition varies on each simulation. The position and rotation of these mobiles parts are used as input to the neural network to obtain the statistics of speed, number of collisions, and traveling time of each agent for this environment and crowd configuration.
% RCB: primeiro foi dito que nenhum trabalho tem o mesmo objetivo... Mas o trabalho acima me parece extremamente relacionado. Correto?
% EST: sim, verdade, me passei dessas descrições quando achamos esse trabalho novo. Ajustei as descrições passadas.

In this work we propose a methodology for estimating the evacuation of crowds over generic modular rooms using neural networks. These rooms can be connected to form bigger and complex environments, and we also propose heuristics to estimate this environment using the data obtained from estimating each room. We make tests using different neural networks models and calculated the accuracy obtained for four estimated parameters.

==> 3_model.tex <==
In this section, we describe in details our proposed approach. First, we present the development of the crowd simulator that is employed to generate data for the learning process. Next, we present the process used to validate that simulator. Finally, we describe our per-room estimation strategy as well as the heuristics to unify the estimated results.

\subsection{Crowd Simulator}

To develop the crowd simulator we make use of \textit{Unity3D} game engine as a platform and implemented agents endowed with the main inherent collective behaviors as referred in the literature: \textit{i)} \textit{goal seeking}, \textit{ii)} \textit{collision avoidance} and \textit{iii)} \textit{Least effort strategy} behaviors, as discussed in \cite{Fruin:1971b,henderson1971statistics,henderson1972sexual,henderson1974fluid,helbing:1997,Still:2000}.

A {\textit{goal seeking} agent means that the agent will move inside the environment in order to arrive at a goal it is seeking. This behavior is simple to implement, just by keeping a goal position for each agent and moving  the agent towards it.

When applying a \textit{Least effort strategy}, the agent will move in trajectories that require less effort, avoiding turns and selecting the shortest paths. 
%This behavior may conflict with the \textit{collision avoidance}, since in most cases it is needed to change its orientation to avoid to collide with others. 
This behavior was implemented using path finding over a \textit{NavMesh}, a network of connected 3D planes which represents the navigable area. The \textit{NavMesh} used was the one native of \textit{Unity3D} platform.

When applying a \textit{Collision avoidance} behavior, the agent will move avoiding physical contact with obstacles and with other agents. %In part, this behavior is implemented using the \textit{NavMesh} to avoid collision with obstacles. 
In order to avoid collisions with other agents we implemented \textit{ORCA} model \cite{ORCA}. \cite{ORCA} is a method for finding the optimal velocity of each agent so that it manages to move through the environment without colliding, it corrects the course of their movements considering each other agent's velocity and position in a future time, reacting preemptively and avoiding possible collisions between them. We used as the optimization velocity for~\textit{ORCA} the direction each agent is following toward its goal on the \textit{NavMesh}. %An example of this collision avoidance can be seen in Figure~\ref{fig:colavoidance}.
% \begin{figure}[htb]
% \centering
%   \subfigure[Agents move in straight line toward their goals. Paths to goals in red.]{\label{fig:path1}\includegraphics[width=0.46\linewidth]{Figs2/agentePathfinding1}}
%  \quad
%  \subfigure[Agents change their paths to avoid collision between them.]{\label{fig:path2}\includegraphics[width=0.46\linewidth]{Figs2/agentePathfinding2}}
%  \subfigure[Agents resume their path toward their goals.]{\label{fig:path3}\includegraphics[width=0.46\linewidth]{Figs2/agentePathfinding3}}

% \caption{Example of \textit{collision avoidance} behavior in a simple environment. (a) Agents move towards their goals in a simple environment. (b) Agents avoiding collision. (c) Agents resume their paths.}     
% \label{fig:colavoidance}
% \end{figure}


%Lastly, we designed simulations to be used to train ANNs. We simulated rooms with 6 following parameters: \textit{Room width}, \textit{Room length}, \textit{Exit size}, \textit{Input flow}, \textit{Flow Duration} and \textit{Initial population}. Also, for each executed simulation we collected the following 
%data needed for calculating the \textit{EP} value parameters: (\textit{Total evacuation time},\textit{Average exit time},\textit{Average speed} and \textit{Average density}). This is going to be detailed in Section \ref{sec:database}. 
As our simulator is going to be used to train and test the ANNs, we considered very important to evaluate its correctness. So, in next sections we describe the validations performed with our simulator.

%SO: tenho dúvidas sobre a próxima section no que tange o paper a ser submetido...
\subsubsection{Model validation}

The validation of our crowd simulation was separated in two steps: evaluate our $ORCA$ implementation when compared to the original one, and validate its similarity with real crowds. 

For the first step the main behavior is the collision avoidance.% and it is illustrated in Figure~\ref{fig:colavoidance}. 
In order to compare with the original ORCA, we recreated one of the~\textit{ORCA}'s showcases available at the developer's website~\cite{ORCAsite}. Some images of this showcase can be seen in Figure~\ref{fig:showcase2}. 

For the real crowd validation we used the same cases used to validate \textit{CrowdSim}~\cite{Cassol:2015} which was based on the \textit{guidelines for evacuation analysis for new and existing passenger ships} proposed by the International Maritime Organization (IMO)\cite{IMO:2007}. This validation is composed of component and qualitative tests. Further details are presented in Section~\ref{sec:IMO}.

%SO: section abaixo diminuir bastante para o paper a ser submetido
\subsubsection{Comparing with \textit{ORCA} showcase}

One showcase was created to show the agents behaviors using \textit{ORCA} to avoid collision and its capacity to move efficiently while looking natural to the human eye. We recreated this showcase only using visual information from real ORCA cases, without knowing the agents parameters (e.g. agents positions or speeds), so we expected similar results but maybe not the same. Nevertheless, a good visual comparison of the behaviors could still be done.

%The first showcase consists of an environment with no obstacles and ten agents positioned in a circular pattern, in which each agent is supposed to move towards the opposing end of the circle, while avoiding collision with the others. As the agents move towards the center, the space between them becomes smaller and some of them will need to assume non-optimal routes and reduce velocities to avoid the collisions. In both implementations (ORCA showcase and ours), agents move successfully towards their goals, reduce their speed and change their courses to avoid collision with others. Both the first showcase and our simulation can be visualized in Figure~\ref{fig:showcase}.

% \begin{figure}[htb]
% \centering
%  \subfigure{\label{fig:orcacase1}\includegraphics[width=0.45\linewidth]{Figs2/validateCase1}}
%  \quad
% \subfigure{\label{fig:orcaval1}\includegraphics[width=0.45\linewidth]{Figs2/validatedCase1}}

%  \subfigure{\label{fig:orcacase3}\includegraphics[width=0.45\linewidth]{Figs2/validateCase3}}
%  \quad
% \subfigure{\label{fig:orcaval3}\includegraphics[width=0.45\linewidth]{Figs2/validatedCase4}}

%  \subfigure{\label{fig:orcacase5}\includegraphics[width=0.45\linewidth]{Figs2/validateCase5}}
%  \quad
% \subfigure{\label{fig:orcaval5}\includegraphics[width=0.45\linewidth]{Figs2/validatedCase5}}

% \caption{Comparison between the \textit{ORCA}'s showcase (left) and our simulation (right). Agents are positioned in a circular pattern and moves to the opposite end of the circle while avoiding collisions with others.}     
% \label{fig:showcase}

% \end{figure}


The showcase consists of 41 agents in three groups, the agents of each group are positioned to form each the letters of the word "RVO". Then they proceed to move down the screen to form the word "UNC". The group forming the letter "R" moves to form the letter "N" at the end of the showcase, the one forming the letter "V" forms the letter "C" and the one from the letter "O" forms the letter "U". Easier movements could be made to complete this transformation, however this specific movement was chosen in order to promote more potential collisions, thus requiring the use of collision avoidance mechanisms, ideal for testing ORCA. A comparison showing the showcase and our simulation as well as the movement pattern generated by both simulators can be visualized in Figure~\ref{fig:showcase2}. In both cases the agents succeeded in moving and forming the other word, in a similar way. %Visually comparing them we say the agents in the showcase had a little more scattered movement pattern, this may be due to the difference in the size of the environment or the difference in the prediction time ORCA uses to make the agents react to the possible collisions. Please, notice, that as we said before we did not know the used parameters, but just imitating the showcases based on visual results.

\begin{figure}[htb]
\centering
 \subfigure{\label{fig:orcacase12}\includegraphics[width=0.47\linewidth]{Figs2/validate2Case1}}
 \quad
\subfigure{\label{fig:orcaval12}\includegraphics[width=0.47\linewidth]{Figs2/validated3Case1}}

 \subfigure{\label{fig:orcacase32}\includegraphics[width=0.47\linewidth]{Figs2/validate2Case3}}
 \quad
\subfigure{\label{fig:orcaval32}\includegraphics[width=0.47\linewidth]{Figs2/validated3Case3}}

 \subfigure{\label{fig:orcacase52}\includegraphics[width=0.47\linewidth]{Figs2/validate2Case5}}
 \quad
\subfigure{\label{fig:orcaval52}\includegraphics[width=0.47\linewidth]{Figs2/validated3Case5}}

\caption{Comparison between the \textit{ORCA}'s showcase (left) and our simulation (right). 41 agents are positioned forming the word "RVO" and moves down the screen to form the word "UNC" while avoiding collisions with others.}     
\label{fig:showcase2}

\end{figure}

\subsubsection{Validation according to IMO}
\label{sec:IMO}

As mentioned before, we propose to validate our simulator using the \textit{guidelines for evacuation analysis for new and existing passenger ships} developed by the International Maritime Organization (IMO)\cite{IMO:2007}. This validation is composed of component and qualitative tests. Component tests are used to check if the tested software performs as intended. Two component tests were conducted: \textit{Maintaining set walking speed} and \textit{Rounding Corners}. Qualitative tests are concerned with the nature of predicted human behavior with informed expectations from observed situations, as they demonstrate the capability of the model to produce realistic behaviors. Three qualitative tests were realized: \textit{Counter flow}, \textit{Exit flow} and \textit{Exit route allocation} tests. They are detailed in next sections.  

\vspace{0.5cm}
\textit{A) Maintaining set walking speed}: This test consists of simulating a single agent moving in a straight line free of obstacles at 1m/s and it is successful if the agent walks 10 meters in 10 seconds. In our simulation the agent succeeded by arriving at the end of the 10 meters corridor at time 9.66 seconds. 

\vspace{0.5cm}
\textit{B) Rounding Corners}: This test evaluates the agent's ability to navigate around a corner without penetrating the walls and without overlapping each other. For this we simulated 40 agents moving towards a goal in a corridor with a 90 degrees turn. The corridor is 2 meters wide with a 10 meters long segment before the turn and another segment after the turn, the area of the turn is a 2x2 meters square. During the test we have detected no agents outside the navigation area, which means no agent penetrated obstacles, and no overlapping between the agents during the turn, so the test was considered a success. An image of the test can be seen in Figure~\ref{fig:casecurve}.


\begin{figure}[htb]
\centering
\subfigure{\label{fig:orcaval1}\includegraphics[width=0.9\linewidth]{Figs2/case_curve}}

\caption{Footage from a group of agents making a turn in the \textit{Rounding Corners} test.}  
\label{fig:casecurve}

\end{figure}

\vspace{0.5cm}
\textit{C) Counter flow}:
This test consists of moving 100 agents between two rooms of 10x10 meters connected by a corridor of 2 meters wide and of 10 meters length. The test is repeated with a counter flow of 10, 50 and 100 agents. The time it takes for the last agent to enter the second room is recorded and it is expected that the time increases as the people on the counter flow increases.  IMO's guidelines for this test can be seen in Figure~\ref{fig:casecounter}. As can be seen in Table~\ref{tab:counterflow}, the recorded time for our simulations increased along with the agents in counter flux, making the test successful.

\begin{figure}[htb]
\centering\subfigure{\includegraphics[width=1\linewidth]{Figs2/counterflow_guide}}

\caption{\textit{Counter flow} scenario configuration, following IMO's specification.}  
\label{fig:casecounter}

\end{figure}

\begin{table}[htb]
\centering
\begin{tabular}{|p{0.3\linewidth}|l|}
\hline
 & \\
Case & Time (seconds) \\  \hline \hline
No counter flux  & 21 seconds \\  \hline
10 counter flux  & 30 seconds \\  \hline
50 counter flux  & 45 seconds \\  \hline
100 counter flux  & 55 seconds \\  \hline
\end{tabular}

\quad

\caption{Time taken for each configuration in the \textit{Counter flow} test.}
\label{tab:counterflow}
\end{table}

\vspace{0.5cm}
%\textit{D) Exit flow}: The environment for this test is a large 30x20 meters room with four exits of 1 meter each, positioned along the 30 meters sides at 4 meters from the walls. 1000 agents are uniformly distributed in a 16x26 region at the center of the room. The simulation is done twice, the second time with the exits on one side closed. The IMO's specification for this scenario is illustrated in Figure~\ref{fig:caseexit}. The elapsed time in the second case should be around 50 percent greater than the first to be successful in this test. In our simulations, the first case computed 41 seconds and the second computed 68 seconds, while at a considerable margin, we can consider the test successful.

% \begin{figure}[htb]
% \centering
% \subfigure{\includegraphics[width=0.99\linewidth]{Figs2/exitflow_guide}}

% \caption{\textit{Exit flow} scenario configuration, following IMO's specification.}  
% \label{fig:caseexit}

% \end{figure}

\vspace{0.5cm}
\textit{E) Exit route allocation}:
This test involves a more complex scenario, a cabin corridor with 12 cabins, two intersecting corridors of different widths, two exits of different sizes and a fixed number of agents according to the cabin. The specification can be seen detailed in Figure~\ref{fig:casecabin}. The criteria for this test is that each agent should move to the closest exit, which means that agents in cabins 1, 2, 3, 4, 7, 8, 9 and 10 should move to the main exit, and the remainder to the secondary exit. In our simulation, the exits were correctly assigned.

\begin{figure}[htb]
\centering
\subfigure{\includegraphics[width=0.99\linewidth]{Figs2/cabin_guide}}

\caption{\textit{Exit route allocation} scenario configuration, following IMO's specification.}  
\label{fig:casecabin}

\end{figure}


\subsection{Estimation of Rooms Parameters based on ANNs}
\label{sec:room_estimation}

Once last sections validate our simulator, this section presents our model to estimate crowd data, resulting of evacuation process, instead of simulating it. As said before we are interested about to test ANN as a tool to estimate crowd parameters instead of generate them through simulation. The overview of our method comprehends three phases: Firstly, we performed several simulations in order to compose the dataset to be used to train the ANN (see Section~\ref{sec:database}). The second phase is responsible for ANN training and validation, as discussed in Section~\ref{sec:trainingmodel}. The third phase is focused on testing the learning methodology for rooms estimation in complex environments (Section~\ref{sec:env_estimator}).
%we The ANN is trained using simulations performed with our simulator w.r.t various configurations of rooms and population, as following described: 
%SuAs a summary of the method we designed for the estimations, it basically sees the environment as a set of modular connected rooms, each room containing its own values of:
The room parameters in our method, as it is designed to compose the dataset to train, validate and test, are following described:

\begin{itemize}
\item \textit{Room width} (meters), 
\item \textit{Room length} (meters), 
\item \textit{Exit size} (meters), 
\item \textit{Input flow} (Agents per second that entry in the room), 
\item \textit{Flow Duration} (Duration in seconds defining the period where agents entry in this room) and 
\item\textit{Initial population} (Number of agents which are inside the room at the beginning of the simulation).
\end{itemize}

Then the estimation proceeds by estimating the following data for each room $i$:

\begin{itemize}
\item \textit{Evacuation total time} $tt_i$ (seconds), 
\item \textit{Average exit time} $\bar{t_i}$ (seconds), 
\item \textit{Average speed} $\bar{s_i}$ (meters per second) and 
\item\textit{Average density} $\bar{d_i}$ (agents per meter).
\end{itemize}
 
%After the data of all rooms were estimated it proceeds by estimating this same data but for the entire environment. This modularization is done to allow us to estimate different environments with different layouts while maintaining the same estimation procedure. 

Details about the estimation procedure is given in next sections.

\subsubsection{Database Creation\label{sec:database}}

To create a database of simulations that could be used to train and test the learning algorithms, we automatized the process of creating rooms. This process generates simulations based on the input parameters, which are randomized for each simulation, and it collects data of the output parameters. Each generated simulation is composed of a rectangular room with a single exit~\footnote{In this paper we investigate specifically the scope of rectangular rooms and single exits. Different rooms geometry and number of exits are going to be addressed in a future work.} The room's dimensions vary according to the \textit{Room width} and \textit{Room length} parameters, the exit size varies according to the \textit{Exit size} parameters. 

Agents are placed in the room using the \textit{Initial population}, \textit{Input flow}  and \textit{Flow Duration}  parameters. The agents informed in initial population are the ones whose are already in the room at the beginning of the simulation.
\blue{They are created and placed in a squared spiral pattern, forming a diamond at the center of the room as more agents are placed, to avoid agents overlapping each other. Figure~\ref{fig:diamond} shows agents placed according to this pattern. As the number of agents rises, the area of the diamond increases. However, as their position are restricted by the size of the room, if no space is available to accommodate all agents that are created, it may be inevitable that some agents will start positioned overlapping others. If this happens agents will try to avoid collisions among them when simulation starts, eventually finding enough space to move without colliding as other agents exit the room.}

\begin{figure}[htb]
\centering
\includegraphics[width=0.75\linewidth]{Figs2/spawn_pattern}
\caption{Agents placed in a squared spiral pattern in a 6x6 room in the crowd simulator, numbered in the order they are placed.}     
\label{fig:diamond}
\end{figure}

New agents $n$ are created w.r.t to flow information. These agents are created at the entrance in the opposite direction of the exit in a room $i$, considering a flow in rate defined as: 

\begin{eqnarray}
n_i = f_i . F_i^t,
\end{eqnarray}
where $f_i$ is the \textit{Input flow} defined for room $i$, and
$F_i^t$ is the \textit{Flow Duration} for $i$ at a time $t$ that is included in the interval $[t_i;t_f]$ that represent respectively initial and final time for the people flow in the room.
When $t$ is greater than $t_f$, i.e. the people flow in room $i$ is finished, $F_i^t=0$, so the entrance of agents in room $i$ stops. 

%Agents always enter into the room from an entrance in the opposite side of the exit.
%SO: frase estranha aqui abaixo | ajustei um pouco
%This entrance size is proportional to the \textit{Input flow}, so that it has necessary space to continuously place new agents without overlapping the ones that were just created moments ago.
%SO: Frase estranha acima... entrance size (meters) é proporcional ao flow? que proporção desejada é essa? Acho melhor comentar a frase acima... Já falamos mais acima que pode ter overlaps temporários... | ok, then ajustei tudo pra ficar direito

In regard of other parameters present during the simulation: the space each agent occupies is represented through a cylinder with a radius of 0.3 meters and it moves trying to maintain a max speed of 1.2 m/s. Both of these values were extracted from the literature for the average value people size and the average speed people have while walking \cite{tilley2002measure}.

\textit{ORCA} makes use of a prediction time to make agents react and avoid collisions with each other. We were not able to find any research or study about which value must be used to be more close to reality. In fact, the common assumption is that value can vary according to each individual (cultural or personality) and with the environment conditions such as time of day, smoke, fire and crowd density. 
\blue{In our simulations we empirically adopted the value of 3 seconds because it was the value which we got better visually convincing collisions avoided during simple tests. When we used prediction time equal to 1 second, the method provided a strange behavior when one agent passes by another one in low densities. In this case, they got too close to each other, while having free space to navigate around. When we used 5 seconds the agents became too much generous, frequently stopping to allow others to pass even from far away distances.}


%SO: fiz uma pequena alteração, veja o que achas.

To generate the training and validation database the room's parameters were randomly defined, in the intervals specified in Table~\ref{tab:values}.
We generated 18000 rooms for training and 2000 for validation. The tests are presented later in Section~\ref{sec:results}.
\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
Parameter & Min value & Max value & Value Type \\ \hline
 \textit{Room width} & 2.0 & 20.0 & Float        \\ \hline
\textit{Room length} & 2.0 & 20.0 & Float        \\ \hline
\textit{Exit size} & 0.9 & 5.0 & Float \\ \hline
\textit{Input flow} & 1.0 & 10.0 & Float \\ \hline
\textit{Flow duration} & 0.2 & 100.0 & Float
\\ \hline
\textit{Initial population} & 0 & 99 & Integer
\\ \hline
\end{tabular}

\quad

\caption{Parameters and values.}
\label{tab:values}
\end{table}


%SO: For 
%The same was made for the testing case, however the case created in the Environment Editor was modeled after a real world case with a real scenario.

\subsubsection{Training and validation\label{sec:trainingmodel}}

\blue{For each attribute to be estimated (Evacuation time, Average exit time, Average speed and Average density) we trained a different neural network, this was done to avoid connecting the learning process of one parameter to the others, as it is possible that a network model works best for one while other model is best for other and that one training could better identify Evacuation Time over Average density and another training the opposite, for example.}
We started with a simple model of neural network: one hidden layer with six neurons fully connected and no bias. The loss function used was the mean squared error function. 
\blue{The training process was made using Stochastic Gradient Descent (SGD), stopping only when no more reduction on the loss was observed by new epochs even when reducing the learning rate.}

\blue{ Vi os tipos de gradiente descendente que tem e na real a gente fez pelo stochastic. }

With these 4 networks trained, the following individual validation errors were measured using the absolute relative error comparing the predicted value and the simulated value. 
We measured the quality of our estimations according to how many cases had less than 10\% error size. %We believe 10\% of error is acceptable to replace a full crowd simulation for a crowd parameters estimation. Moreover, we do not have any reference to compare what is a good estimation in terms of crowd evacuation, since we did not find such information in literature.
%SO: acrescentei uma justificativa

The Evacuation time estimated by the ANN resulted in 89.5\% of the validation cases bellow 10\% error, the Average exit time presented 72.3\% of the cases, while the Average speed and Average density networks presented 40.9\% and 45.7\% respectively. The errors histograms of these networks can be seen in Figures \ref{fig:ST6neurons}, \ref{fig:AE6neurons}, \ref{fig:AS6neurons} and \ref{fig:AD6neurons}.

\begin{figure}[htb]
\centering
\includegraphics[width=1\linewidth]{Figs/6Simulation_time__seconds_.png}
\caption{Hidden layer with 6 neurons, Total evacuation time error percentage.}     
\label{fig:ST6neurons}
\end{figure}

\begin{figure}[htb]
\centering
\includegraphics[width=1\linewidth]{Figs/6Average_exit_time__seconds_.png}
\caption{Hidden layer with 6 neurons, average exit time error percentage.}     
\label{fig:AE6neurons}
\end{figure}

\begin{figure}[htb]
\centering
\includegraphics[width=1\linewidth]{Figs/6Average_speed__m_s_.png}
\caption{Hidden layer with 6 neurons, average speed error percentage.}     
\label{fig:AS6neurons}
\end{figure}

\begin{figure}[htb]
\centering
\includegraphics[width=1\linewidth]{Figs/6Average_density.png}
\caption{Hidden layer with 6 neurons,average density error percentage.}     
\label{fig:AD6neurons}
\end{figure}



%Despite our main objective being the creation of a methodology to allow the estimation of entire environments and not exactly the search for the best network to do so, we still searched for a better model. 
In order to test other ANNs architectures, we perform a variation in the quantity of neurons on the hidden layer and evaluating the results. New attempts were made using 50, 200, 400 and 500 neurons on the hidden layer. Each attempt efficiency was measured by collecting how many cases during individual validation were bellow 10\% error size, as it can be seen in Figure~\ref{fig:treinamentos}. 

The best configuration obtained for each attribute was with 400 neurons for the Evacuation time and for Average exit time and 200 neurons for Average density. Average speed had nearly the same result with 200 and 400 neurons, but 200 neurons was chosen because of its slightly smaller standard deviation during individual validation. With these new ANN configurations, the number of cases bellow 10\% error improved for all attributes: from 89.5\% to 91.5\% in Evacuation time, from 72.3\% to 85.4\% in Average exit time, from 40.9\% to 49.9\% in Average speed and from 45.7\% to 51.6\% in Average density. The error histograms can be seen in Figures \ref{fig:ST400neurons}, \ref{fig:AE400neurons}, \ref{fig:AS200neurons}, \ref{fig:AD200neurons}. As could be seen, our tests indicate that evacuation and average exit times are parameters that seem to be adequate to be used in such type of ANNs. Fortunately, although the other parameters are also important, these two related to the time are more important in evacuation scenarios evaluation. That is the reason why we pursue our investigation using only these two attributes and keeping densities and velocities for a next work.

Next section describes our heuristic capable of aggregating per-room information in order to estimate complex environments.

\begin{figure}[htb]
\centering
\includegraphics[width=1\linewidth]{Figs/scattertraining.png}
\caption{Search for a better network model. Attempts with 6, 50, 200, 400 and 500. Plotted number of cases bellow 10\% error in the individual validation.}     
\label{fig:treinamentos}
\end{figure}

\begin{figure}[htb]
\centering
\includegraphics[width=1\linewidth]{Figs/400_neurons_-Simulation_time__seconds_.png}
\caption{Hidden layer with 400 neurons, Total evacuation time error percentage.}     
\label{fig:ST400neurons}
\end{figure}

\begin{figure}[htb]
\centering
\includegraphics[width=1\linewidth]{Figs/400_neurons_-Average_exit_time__seconds_.png}
\caption{Hidden layer with 400 neurons, average exit time error percentage.}     
\label{fig:AE400neurons}
\end{figure}

\begin{figure}[htb]
\centering
\includegraphics[width=1\linewidth]{Figs/200_neurons_-Average_speed__m_s_.png}
\caption{Hidden layer with 200 neurons, average speed error percentage.}     
\label{fig:AS200neurons}
\end{figure}

\begin{figure}[htb]
\centering
\includegraphics[width=1\linewidth]{Figs/200_neurons_-Average_density.png}
\caption{Hidden layer with 200 neurons,average density error percentage.}     
\label{fig:AD200neurons}
\end{figure}

%SO: aqui abaixo acho que vai apra results

% Validating these new networks with the environments cases, figure \ref{fig:400-400-200-200}, improvements in the Simulation time, Average speed and Average density can be observed, from 22\% average error to 19\%, 61\% to 52\% and 53\% to 46\% respectively, while maintaining basically the same standard deviation. Average exit time suffered from 65\% to 71\%, keeping the same standard deviation.

% \begin{figure}[htb]
% \centering
% \includegraphics[width=1\linewidth]{Figs/400-400-200-200_average.png}
% \caption{Validation of estimated environments with 14 environment cases using networks with 400 hidden neurons for Simulation time and Average exit time and 200 neurons for Average speed and Average density. The average error and standard deviation of each attribute is shown.}     
% \label{fig:400-400-200-200}
% \end{figure}

\subsection{Environment Estimation based on ANNs and Heuristics}
\label{sec:env_estimator}

As described in last section, the crowd data to estimate the evacuation times at each room uses ANNs. %, four of them focused on learning specific crowd parameters, i.e. Simulation time, Average exit time, Average speed and Average density. 
However, in general, crowd evacuation methods are used for more complex environments than only one room. Therefore, 3D modeling is usually necessary in order to create the environment to be simulated. Once we are proposing a crowd estimation instead of simulation, we propose to create a simple environment based on a graph of rooms (i.e. an environment graph where the connections among the rooms are defined as graph edges). We developed an environment editor (see Section~\ref{sec:EnvEditor}), where the user can easily create and edit a graph representing an environment to be estimated. 

Our proposal is to use ANNs to estimate the parameters from each room (as discussed in last section) and then combine this data, through an empirically defined heuristic to compute the global data for the whole environment. Heuristics are used in two phases. The first one is responsible for considering the hierarchy of rooms adjusting the population and flows of rooms that lead people to other rooms. Then, in a second step, the global data regarding the whole environment is computed.

%For each data to be estimated in the room a neural network is trained, it receives the values of the rooms as input to estimate the resulting data of the room. 
One environment $e$ is composed by $N$ rooms $r$ to be estimated. We estimated the crowd parameters at each $r_i$, tested with the two specific ANNs, one for each crowd parameter ($tt_i$ and $\bar{t_i}$), as previously specified. Therefore, we have two types of rooms $r$ in an environment $e$: \textit{i)} rooms of type $D$ which population impacts another room, i.e. people from $r_{D_i}$ comes to another $r_i$ and \textit{ii)} rooms of type $E$ (exit rooms) which are rooms that lead the population to the output of the environment. Moreover, these two types of rooms are exclusive, i.e. rooms $D$ never lead to exit and $E$ rooms never impact any other room in $e$. %The details about the training of those neural networks are present on chapter \ref{sec:results}.

\vspace{0.5cm}
\noindent\textit{A~-~The Heuristics to Estimate each Room}
\vspace{0.5cm}

The environment estimator loads the specified environment (using the Editor as defined in Section~\ref{sec:EnvEditor}) and performs the data estimation for each room separately (types $D$ and $E$) using the two specific ANNs (as described in Section~\ref{sec:room_estimation}). Obtained data for room $r_i$ are: \textit{Evacuation total time} ($tt_i$) and \textit{Average exit time} ($\bar{t_i}$).
%\textit{Average speed} ($\bar{s_i}$) and \textit{Average density} ($\bar{d_i}$). 
As said before, some rooms have dependence rooms, i.e. a certain $r_i$ is impacted by other rooms (type $D$) which population goes to $r_i$. This is the definition of the set of $r_{D_i}$ dependence rooms that impact $r_i$. That is the reason why some rooms have to be estimated before others. So, firstly we are going to present the execution flow for rooms which do not have dependence ($N_{D_i}=0$), i.e. first rooms in the environment graph.

%The execution flow for each room $r_i$ is following described in five steps:
\begin{enumerate}
%\item {To compute $D_i$, i.e. the dependence rooms of $r_i$};
\item Since no people enters this room coming from another room: \textit{Input flow} $f_i=0$ and \textit{Flow Duration} $F_i=0$,  
%\item \textit{Initial population} $pop_i = ip_i$, % ip_i só é mencionado depois

\item %Having the needed data in place for $r_i$ (room width, room length, exit size, initial population $pop_{i}$ - these four coming from the Environment Editor - Input flow $f_{i}$ and Flow duration $F_{i}$) the estimation of $r_{i}$ can happen. 
The neural networks are loaded and the two output parameters of the room ($tt_{i}$ and  $\bar{t_{i}}$) %, $\bar{s_{i}}$ and $\bar{d_{i}}$) 
are estimated using their respective networks. In addition to these estimations, two other features are computed $fet$ and $gfet$, as follows:


%\begin{eqnarray}
 %fet_{i} = max(0,\bar{t_{i}} - \frac{(tt_{i} - \bar{t_{i}})}{\delta}), 
 %fet_{i} = \frac{length_{i}}{maxSpd}
 %\label{eq:fet}
 %\end{eqnarray}
 
 %\begin{eqnarray}
 %fet_{i} = \frac{\frac{length_{i}}{2} - Max(0,(\frac{0.6 * \sqrt{ip_{i} * 2 - 1}}{2})}{maxSpd} ,
%\label{eq:fet2}
%\end{eqnarray}

 \begin{eqnarray}
 fet_{i} = 
 \begin{cases}
     \frac{length_{i}}{maxSpd},& ip_{i} = 0 \\
     \frac{\frac{length_{i}}{2} - Max(0,(\frac{0.6  \sqrt{ip_{i} . (2 - 1)}}{2})}{maxSpd},              & \text{otherwise}
 \end{cases}
 \label{eq:fet}
 \end{eqnarray}


where $fet_{i}$ is the first exit time from $r_i$ which means the time that the first agent exits such room and $ip_{i}$ is the number of agents initially created in room $i$. It is simply calculated as the time it takes for an agent to pass through the room at maximum speed on the simulator ($1.2m/s$). However, when $ip_{i} > 0$, the first agent to exit will not need to travel all the room length to exit since it will be placed at the center of the room. To deal with that we designed the second part of~Equation~\ref{eq:fet}, which represents the distance reduction  to be traveled by the first agent to exit the room. The next equation is also computed afterwards the ANN execution:

\begin{eqnarray}
 gfet_i = fet_i,
\label{eq:it}
\end{eqnarray}

where $gfet_i$ is the time the first agent exited the room in a global time among all rooms. In the case of rooms without dependence is exactly the value of $fet_{i}$ since they are the ones that "start" the crowd movement in the estimation. %$maxSpd$  is the maximum speed an agent .
Therefore, $fet_{i}$ and $gfet_{i}$ are used to propagate values to the input of rooms that are their dependents.%, and $\delta$ is a value empirically defined as $2.4$.
\end{enumerate}

% \item {If $D_i<>0$ then Estimate(all $r_{D_i}$)}:

% \subitem {Having needed data in place for $r_{D_i}$ (room width, room length, exit size - three coming from the Environment Editor - Input flow $f_{D_i}$, Flow duration $F_{D_i}$ and initial population $pop_{D_i}$) the estimation of $r_{D_i}$ can happen. The neural networks are loaded and each output parameter ($st_{D_i}$, $\bar{t_{D_i}}$, 
% $\bar{s_{D_i}}$ and 
% $\bar{d_{D_i}}$) is estimated using its respective network. In addition, other features are computed:

% \begin{eqnarray}
%  fet_{D_i} = min(at_{D_i}+fet_{D_i}),
% \label{eq:it}
% \end{eqnarray}

% \begin{eqnarray}
%  it_{D_i} = min(at_{D_i}+fet_{D_i}),
% \label{eq:it}
% \end{eqnarray}
% }

For each room $r_i$ which $N_{D_i}>0$ we perform the following execution flow:

\begin{enumerate}
\item {If the room has a dependence ($r_{D_i}$) that is not estimated yet, the estimation of this room is postponed until all dependences are estimated. If all ($r_{D_i}$) are already estimated then we compute the following data for $r_i$}: %If not, $r_i$ estimation should wait untilthis room estimation should be postponed until its dependences are computed.}
%\item {If all dependencies are already estimated then collect their data to attribute to the \textit{Input flow} $f_r$ and \textit{Flow Duration} $F_r$ input parameters for room $r$, as follows:
\subitem 
\begin{eqnarray}
 git_i = min(gfet_{D_i}), \\
 ift_i = max(gfet_{D_i} - fet_{D_i} + st_{D_i}),
\label{eq:iit}
\end{eqnarray}

where $git_i$ is the global initial time of $r_i$, i.e. the time this room receives its first agent coming from a $r_{D_i}$ in a global time among the rooms, and $ift_i$ is the income final time of $r_i$, i.e. the global time the last agent coming from a $r_{D_i}$ enters into $r_i$. These two variables together determines a window in time in which the dependence rooms of $r_i$ will send agents to $r_i$, as described in Equation~\ref{eq:flowduration1}. The input flow is determined as Equation~\ref{eq:flowduration2}. This way all agents coming into $r_i$ from its dependences are considered a constant flux of agents during the time window.
\begin{eqnarray}
 F_i = ift_i - git_i.
\label{eq:flowduration1}
\end{eqnarray}
\begin{eqnarray}
f_i = \frac{\sum_{i=1}^{N_{D_i}} (pop_i  .  in^i_{D_i})}{F_i},
\label{eq:flowduration2}
\end{eqnarray}
where $N_{D_i}$ is the number of dependence rooms of $i$. $in^i_{D_i}$ is the percentage of agents from $D_i$ that goes to $r_i$. $pop_i$ is the population of $r_i$, and it is computed as follows:
\begin{eqnarray}
pop_i = ip_i + (f_i. F_i),
\label{eq:pop}
\end{eqnarray}
where $ip_i$ is the number of agents initially created in room $i$.


\item {%With all the needed data in place for $r_i$ (room width, room length, exit size - three coming from the Environment Editor - Input flow $f_i$, Flow duration $F_i$ and initial population $pop_i$ - calculated as recently explained) the estimation of $r_i$ can happen. 
With all the data needed from dependences propagated in room $i$,
the neural networks can estimate the output parameters of such room ($tt_i$ and $\bar{t_i}$),%, $\bar{s_i}$ and $\bar{d_i}$) 
just as before.} 
\end{enumerate}

The parameter $gfet_i$ is then calculated as follows:
\begin{eqnarray}
 gfet_i = fet_i + git_i.
\label{eq:acctime}
\end{eqnarray}
Equation~\ref{eq:acctime} is different from~\ref{eq:it} because in the first case room $i$ has $N_{D_i}<>0$, i.e. this room has dependences. Consequently, agents pass arrive this room coming from another one, so the time it takes to the first one to exit has an offset of the time it took for someone to enter $r_i$. In the second case, $N_{D_i}=0$, agents start to be simulated in time $=0$.

After we finish the estimation of a certain $r_i$ this whole process is repeated until all $N$ rooms in the environment are estimated. It is important to emphasize that these simple equations have the only goal to aggregate the flow of population passing through the rooms and the global times. Next section presents how such information is used to estimate the whole environment.

%Other equations to aggregate could also be possible, we tested some but at the end these bunch of equations had the better results.

\vspace{0.5cm}
\noindent\textit{B~-~Final Estimation Data Regarding the Environment}
\vspace{0.5cm}

The last step of the environment estimation is to estimate the crowd parameters for the whole environment based on the rooms estimation.
%To summarize all the rooms estimations into a single environment estimation
We first consider the exit rooms data (type $E$) to estimate the  \textit{Evacuation total time} $tt_e$ of a specific environment $e$. Indeed, this is the greatest Total evacuation time of $M$ existent exit rooms that represent the exits in the environment, computed as Equation~\ref{eq:st}:

\begin{eqnarray}
 %st_e = max(at_{E_e}),  
 tt_e = max(git_{E_e} + tt_{E_e}),  
\label{eq:st}
\end{eqnarray}
where $E_e$ are the exit rooms of the environment $e$. The \textit{Average exit time} $\bar{t_e}$ of the environment is the average between the $M$ exit rooms exit time plus the average time agents enter this exit room, as Equation~\ref{eq:totaltime}: 

\begin{eqnarray}
 \bar{t_e} = \frac{\sum_{er=1}^{M}(\bar{t}_{E_{er} + \frac{(git_{er} + ift_{er})}{2}})}{M}.
\label{eq:totaltime}
\end{eqnarray}

%For the \textit{Average speed} $\bar{s_e}$ of the environment $e$ we first get the total estimated population $pop_e$, which is the sum of population estimated at each room:


% \begin{eqnarray}
% pop_e = \sum_{i=1}^{N} pop_i,
% \label{eq:acctime}
% \end{eqnarray}
%\begin{eqnarray}
%pop_e = \sum_{er=1}^{M} pop_{E_er},
%\label{eq:acctime}
%\end{eqnarray}
%where $N$ is the number of rooms in the environment $e$. 
%Then we get $\bar{s_e}$ using the Equation~\ref{eq:speed} %by getting the $\bar{s_r}$:%  of all rooms weighted by its total estimated population: 
% For the \textit{Average speed} of the environment $\bar{s_e}$ we use average of the \textit{Average speed} estimated for each $r_i$:

% \begin{eqnarray}
% \bar{s_e} =\frac{\sum_{i=1}^{N} \bar{s_i}}{N}. %. \frac{pop_i}{pop_e}.
% \label{eq:speed}
% \end{eqnarray}


% Similarly we compute the \textit{Average density} of the environment $\bar{d_e}$ average of the \textit{Average density} obtained for each $r_i$: 

% \begin{eqnarray}
% \bar{d_e} =\frac{\sum_{i=1}^{N} \bar{d_i}}{N}. %. \frac{pop_i}{pop_e}.
% \label{eq:dens}
% \end{eqnarray}

This is the 2d vector containing estimated data for a certain environment $e$ we called $ \vec{ED_e} = \{ tt_e, \bar{t_e}
%, \bar{s_e}, \bar{d_e} 
\}$. We used $\vec{ED_e}$ to compare with $\vec{SD_e}$, resulting from the simulation process, as discussed in Section~\ref{sec:results}.


% \subsubsection{Environment Estimation}\label{sec:estimate}

% To realize these estimations we separated the procedure in two: a environment editor tool to help defining an environment to be estimated and its rooms; and an application that performs the environment estimation for a specific given environment. The tool was developed using the Windows Forms framework, and the application uses a console application in C\#, which receives the file defining the environment by command line.


\subsubsection{Environment editor}
\label{sec:EnvEditor}

The Environment editor is a simple graphical application to allow users to easily create and edit environments to be used for estimation. It consists of a main window divided in two regions, the control panel and the canvas, as shown in Figure~\ref{fig:EEE}. The control panel provides a file menu with options to save the current environment into a file, load an environment from a file and to clear the current environment. Also it has a list of available tools  and a button to add a new room to the current environment.

\begin{figure}[htb]
\centering
\includegraphics[width=1\linewidth]{Figs2/EEE}
\caption{Environment editor main window, control panel and canvas regions and a room are highlighted in red, black arrows indicate each rooms connections to the others.}
\label{fig:EEE}
\end{figure}

The tools available can be used to: \textit{i)} move a room in the canvas in order to locate and organize it as the user wants; \textit{ii)} create a connection from one room to another, indicating that the agents from the first room will move towards the second one; and \textit{iii)} remove an existing room, together with its connections. 

It is also possible to select a room and check its parameters. In this case, a new window will appear, as in Figure~\ref{fig:EEE2}, showing the \textit{Room width}, \textit{Room length}, \textit{Exit size} and \textit{Initial population} parameters along with the connections presented in the selected room. The value of the parameters can be modified by the user and the connections may be removed. %The remaining input parameters, \textit{Input flow} and \textit{Flow duration}, are not present here because they are calculated during the estimation of the environment, based on the rooms connections and estimation results.

\begin{figure}[h]
\centering
\includegraphics[width=0.6\linewidth]{Figs2/EEEvalues}
\caption{Environment editor's room values window, it shows the values of the parameters of the selected room for the user to modify it to design the environment.}
\label{fig:EEE2}
\end{figure}


%SO: puxei esta section psra cima
% \subsubsection*{Estimator application}

% To perform the estimation of each room we make use of a neural network model. For each data to be estimated on the room a neural network is trained, it receives the values of the rooms as input to estimate the resulting data of the room. We have two main types of rooms in an environment $e$: \textit{i)} rooms $r$ which population impacts another room, i.e. people from $r$ comes to another $r$ and \textit{ii)} exit rooms $er$ which are rooms which lead the population to the output of the environment. i.e. it does not impact any other room. The details about the training of those neural networks are present on chapter \ref{sec:results}.

% The estimator application then loads the specified environment and performs the data estimation for each room (types $r$ and $er$) using neural networks. Generated data for room $r$ are: \textit{Simulation time} $st_r$, \textit{Average exit time} $\bar{t_r}$, 
% \textit{Average speed} $\bar{s_r}$ and 
% \textit{Average density} $\bar{d_r}$. In addition, all rooms have an extra output we called \textit{Accumulated time} $at_r$. It is computed based on the $at_r$ for all $r$ dependence rooms, as Equation~\ref{eq:acctime}:
% \begin{eqnarray}
%  at_r = st_r + min(at_d),%|d~is~[0;D_r],
% \label{eq:acctime}
% \end{eqnarray}
% where $at_d$ is the accumulated time for dependence room $d$ of $r$ and function $min$ returns the smaller accumulated time among all dependence rooms $D_r$. If $r$ has not dependences, then $at_r = st_r$. Equations~\ref{eq:min} and~\ref{eq:max} define $min$ and $max$ functions, respectively.

% \begin{eqnarray}
% min(x) = \{x \mid \forall x': x < x'\}.
% \label{eq:min}
% \end{eqnarray}
% % TO DO: aqui que tem que ajustar com o first exit time
% \begin{eqnarray}
% max(x) = \{x \mid \forall x': x > x'\}.
% \label{eq:max}
% \end{eqnarray}

% The execution flow is following described for each room $r$ in four steps:

% \begin{enumerate}
% \item {If a room $r$ does not have dependences, then \textit{Input flow} $f_r$ and \textit{Flow Duration} $F_r$ are null. Then, proceed to step 4)}.
% \item {Verify if all dependencies of $r$ are already estimated. If not, this room estimation should be postponed until its dependences are computed.}
% \item {If all dependencies are already estimated then collect their data to attribute to the \textit{Input flow} $f_r$ and \textit{Flow Duration} $F_r$ input parameters for room $r$, as follows:
% \subitem 
% \begin{eqnarray}
%  F_r = max(at_d) - min(at_d).
% \label{eq:flowduration}
% \end{eqnarray}
% \begin{eqnarray}
% f_r = \frac{\sum_{d=1}^{D_r} pop_d}{F_r},
% \label{eq:flowduration}
% \end{eqnarray}
% where $D_r$ is the number of dependence rooms $d$ of $r$. $pop_d$ is the population of room $d$, and it is computed as follows:
% \begin{eqnarray}
% pop_r = ip_r + (f_r. F_r),
% \label{eq:pop}
% \end{eqnarray}
% where $ip_r$ is the number of agents initially created in room $r$.
% }

% \item {With all the needed data in place the estimation can finally occurs, the neural networks are loaded and each output value is estimated using its respective network.}
% \end{enumerate}

% This process is repeated until all rooms are estimated, skipping the rooms which were already estimated. 

% %To summarize all the rooms estimations into a single environment estimation
% We firstly consider the exit rooms $er$ to estimate the  \textit{Simulation time} $st_e$ of a specific environment $e$. Indeed, this is the greatest 
% accumulated time of $E$ exit rooms that represent the exits in the environment, computed as Equation~\ref{eq:st}:

% \begin{eqnarray}
%  st_e = max(at_{er}),  
% \label{eq:st}
% \end{eqnarray}
% where $er$ are the exit rooms of the environment. %is the estimated time in room $r$, $D_r$ is the number of rooms which agents go to $r$ and $t_d$ is the estimated time in such rooms.
% %$ST_{A}$ = simulated time of room $A$, and$D_{k}^{A}$ = dependency $k$ of room $A$.
% %SORAIA: não entendi a equação acima :( fiz uma versão


% The \textit{Average exit time} $\bar{t_e}$ of the environment is the average between the exit rooms accumulated time. 

% \begin{eqnarray}
%  \bar{t_e} = \frac{\sum_{er=1}^{E}(at_{er})}{E},
% \label{eq:acctime}
% \end{eqnarray}

% For the \textit{Average speed} $\bar{s_e}$ of the environment $e$ we first get the total estimated population $pop_e$, which is the sum of population estimated at each room:

% \begin{eqnarray}
% pop_e = \sum_{r=1}^{N} pop_r,
% \label{eq:acctime}
% \end{eqnarray}
% where $N$ is the number of rooms in the environment $e$. Then we get $\bar{s_e}$ using the Equation~\ref{eq:speed} %by getting the $\bar{s_r}$:%  of all rooms weighted by its total estimated population: 

% \begin{eqnarray}
% \bar{s_e} =\sum_{r=1}^{N} \bar{s_r} . \frac{pop_r}{pop_e}.
% \label{eq:speed}
% \end{eqnarray}


% Finally, similarly we compute the \textit{Average density} $\bar{d_e}$ of the environment: 

% \begin{eqnarray}
% \bar{d_e} =\sum_{r=1}^{N} \bar{d_r} . \frac{pop_r}{pop_e}.
% \label{eq:dens}
% \end{eqnarray}

%TO DO: ajustar a finaleira do processo, Soraia tinha mencionado deixar o EP de lado for now...


%\subsubsection{$EP$ evaluation}

% Finishing the whole process, we feed the estimated values of the environment to the $EP$ metric~\cite{Cassol2017}, as shown in Equation~\ref{eq:avaliacao}:

% \begin{equation}
% \label{eq:avaliacao}
% EP_e = \frac{4}{\frac{1}{st_e}+\frac{1}{\bar{t_e}} + \frac{1}{\bar{d_e}}+ \frac{1}{\bar{s_e}}}. 
% \end{equation}

% So, $EP_e$ aims to measure the quality of a certain evacuation plan that has been estimated in one specific environment. In order to have another evacuation plan we just need to reparametrize  $f_r$ according to the existent bifurcations in the environment. It has been implemented but not tested in a full environment.


%TO DO: ajustar com os dados do database atual
% \subsubsection{Database Creation\label{sec:database}}

% To create a database of simulations that could be used to train and test the learning algorithms, we automatized the process of creating rooms. This process generates simulations based on the input parameters, which are randomized for each simulation, and it collects data of the output parameters. Each generated simulation is composed of a square room with a single exit. The room's dimensions vary according to the \textit{Room width} and \textit{Room length} parameters, the exit size vary according to the \textit{Exit size} parameters. 

% Agents are placed in the room using the \textit{Initial population}, \textit{Input flow} and \textit{Flow Duration} parameters. Such agents are created at the beginning of the simulation in a diamond pattern at the center of the room to avoid agents overlapping to each other. However, as they position is restricted by the size of the room, if no space is available to accommodate all of agents that need to be created, it may be inevitable that some agents will start positioned overlapping others. 

% New agents $n_r$ are created to enter the room $r$ in a rate defined as: 

% \begin{eqnarray}
% n_r = f_r . F_r^t,
% \end{eqnarray}
% where $f_r$ is the \textit{Input flow} defined for room $r$, and
% $F_r^t$ is the \textit{Flow Duration} for $r$ at a time $t$ that is included in the interval $[t_i;t_f]$ that represent respectively initial and final time for the people flow in the room.
% When $t$ is greater than $t_f$, i.e. the people flow in room $r$ is finished, $F_r^t=0$, so the entrance of agents in room $r$ stops. 

% Agents always enter in the room from an entrance in the opposite side of the exit.
% The entrance size is proportional to the \textit{Input flow}, so it has necessary space to continue creating new agents while avoiding to place it overlapping the ones that were just created.

% For the other parameters, the space each agent occupy is represented with a cylinder with a radius of 0.3 meters and they move trying to keep at a max speed of 1.2 m/s. Both of these values were extracted from the literature for the average value people occupy and the average speed people have while walking \cite{tilley2002measure}.

% As for the preemptive time \textit{ORCA} used to make agents react and avoid collisions, we were not able to find any research or study about which value must be used to be more close to reality. In fact, the common assumption is that value can vary according to each individual (cultural or personality) and with the environment conditions such as time of day, smoke, fire or even crowd density. In our simulations we adopted the value of 3 seconds because it is the value we empirically obtained better results during a set of tests.

% With these simulations we generated a database of 18.087 simulations. Its parameters were randomly defined, in the intervals specified in Table\ref{tab:values}. 
% \begin{table}[h]
% \centering
% \begin{tabular}{|c|c|c|c|}
% \hline
% Parameter & Min value & Max value & Value Type \\ \hline
%  \textit{Room width} & 2.0 & 20.0 & Float        \\ \hline
% \textit{Room length} & 2.0 & 20.0 & Float        \\ \hline
% \textit{Exit size} & 0.9 & 5.0 & Float \\ \hline
% \textit{Input flow} & 1.0 & 10.0 & Float \\ \hline
% \textit{Flow duration} & 0.2 & 100.0 & Float
% \\ \hline
% \textit{Initial population} & 0 & 99 & Integer
% \\ \hline
% \end{tabular}

% \quad

% \caption{Parameters and values.}
% \label{tab:values}
% \end{table}


==> 4_training.tex <==
This section describes some results we obtained testing our method. Section~\ref{sec:part1} describes experimental results when simulating and estimating 20 full scenarios with varied population distribution in the rooms. In Section~\ref{sec:Part2} we modeled 30 new environments by replicating rooms and evaluated them in order to measure the impact of ANN error. Finally, we proceed with a practical usage of our method applying it in a real life environment.


% which comprises the usage of ANNs to estimate data in specific rooms, and proposed heuristics to merge the rooms into a complete environment. 
%The tool was developed using the Windows Forms framework, and the application uses a console application in C\#, which receives the file defining the environment by command line.
%As said before, 
%We used a dataset of 18000 rooms for training and 2000 for validating each ANN used.
\subsection{Evaluating Environments with Varied Populations}
\label{sec:part1}

For the first set of scenarios to be tested, we created some full varied environments to be estimated and simulated. Our goal is to show the obtained errors when comparing our method for estimation with the full simulation execution.

Firstly, using the Environment Editor, we have manually created 10 environments to be tested in our method using the application illustrated in Figure~\ref{fig:EEE}. These cases are composed of a set of consecutive rooms, each one with its own width, height and exit size. In order to simulate those environments, we used our simulator developed at Unity. Figure~\ref{fig:salas} shows an example of an environment modeled using Unity Engine (on the left) and in the Environment Editor (on the right).

\begin{figure}[htb]
\centering
 \subfigure{\includegraphics[width=0.40\linewidth]{Figs/5_salas_unity}}
 \quad
\subfigure{\fbox{\includegraphics[width=0.52\linewidth]{Figs/5_salas_editor}}}

\caption{Example of an environment case: five consecutive rooms with different exit sizes. On the left: the environment at Unity, and on the right in the Environment Editor.}
\label{fig:salas}

\end{figure}

For each of those environments the initial population is placed in the first rooms of the environment (the ones with no dependencies), in the graph that represents the environment, and move to the exit (last room). In a next step we simulate and estimate each environment with same number of agents ($3^{rd}$ column in the table) and collect results information. Results are shown in Figure~\ref{fig:err_val}, that contain respectively the percentage relative error of total evacuation time ($tt$) and average time per agent ($\bar{t}$) when compared to the values achieved in the simulations. These 10 simulations were named $Sim_i$, where $i$ is in the interval $[1;10]$.

Additionally, we created 10 new cases by copying these previous 10 w.r.t the environment geometry and number of agents, but varying the population distribution among the other rooms as well, i.e. in those cases agents are not initially placed only in the first room in the environment. We named these simulations as $Sim_i'$, having also $i$ in the interval $[1;10]$. We used the same distribution in the simulation data and proceed again with estimations and simulations. In the same way we compute the percentage relative error when compared with the simulations. Figure \ref{fig:salasmodeled} shows the 10 scenarios created on the crowd simulator and used for these 20 cases.

\begin{figure}[htb]
\centering
\includegraphics[width=1\linewidth]{Figs/AnaliseSoraia.png}
\caption{Obtained results when testing 20 environments. The percentage of errors are shown for total evacuation time $tt_e$ and for average time $\bar{t}_e$ metrics for each environment.}     
\label{fig:err_val}
\end{figure}

\begin{figure*}[hbt]
\centering

\subfigure[Sim 1]{\includegraphics[scale=0.15]{Figs/2_routes}}
\quad
\subfigure[Sim 2]{\includegraphics[scale=0.165]{Figs/3_rooms_widening_exit}}
\quad
\subfigure[Sim 3]{\includegraphics[scale=0.175]{Figs/Teste_3-1_saida}}

\subfigure[Sim 4]{\includegraphics[scale=0.16]{Figs/Teste_4_salas}}
\quad
\subfigure[Sim 5]{\includegraphics[scale=0.1]{Figs/Teste_5_corredor}}
\quad
\subfigure[Sim 6]{\includegraphics[scale=0.15]{Figs/4_small_rooms}}
\quad
\subfigure[Sim 7]{\includegraphics[scale=0.14]{Figs/Teste_5_salas_funil}}

\subfigure[Sim 8]{\includegraphics[scale=0.15]{Figs/5_identical_rooms}}
\quad
\subfigure[Sim 9]{\includegraphics[scale=0.155]{Figs/7_identical_rooms}}
\quad
\subfigure[Sim 10]{\includegraphics[scale=0.15]{Figs/9_identical_rooms}}

\caption{Scenarios modeled in the crowd simulator for the 20 cases for evaluating environments with varied population.}
\label{fig:salasmodeled}

\end{figure*}

%For each of those environments (named in $1^{st}$ column and illustrated in $2^{nd}$ of Table~\ref{tab:env_err}), the initial population is placed in the first rooms of the environment (the ones with no dependencies), in the graph that represents the environment, and move to the exit (last room). In a next step we simulate and estimate each environment with same number of agents ($3^{rd}$ column in the table) and collect results information. Results are shown in Table~\ref{tab:env_err}, in $4^{th}$ and $5^{th}$ columns, that contain respectively the percentage relative error of total evacuation time ($tt$) and average time per agent ($\bar{t}$) when compared to the values achieved in the simulations. These 10 simulations were named $Sim_i$, where $i$ is in the interval $[1;10]$.

%Additionally, we created 10 new cases by copying the previous 10 (from Table~\ref{tab:env_err}) w.r.t the environment geometry and number of agents, but varying the population distribution among the other rooms as well, i.e. in those cases agents are not initially placed only in the first room in the environment. We named these simulations as $Sim_i'$, having also $i$ in the interval $[1;10]$. We used the same distribution in the simulation data and proceed again with estimations and simulations. In the same way we compute the percentage relative error when compared with the simulations (results presented in $6^{th}$ and $7^{th}$ columns).

% \begin{table*}[!htpb]
% \centering
% \caption{Environment cases configuration and estimation relative errors.}
% \begin{tabular}{|c|c||c|c|c||c|c|}
% \hline
% Case ID & Environment & Population &  $tt$ when agents  & $\bar{t}$ when agents & $tt$ when agents & $\bar{t}$ when agents \\ 
%  & Shape &  &  only in $r_1$ & only in $r_1$  & distributed in $e$  & distributed in $e$ \\ \hline
% Sim 1 & \includegraphics[scale=0.1]{Figs/2_routes}  			& 20 agents & -29\% & -15\% 	& -2\% 	&  25\% \\ \hline
% Sim 2 & \includegraphics[scale=0.1]{Figs/3_rooms_widening_exit} & 20 agents & -31\% & -17\% 	& -5\% 	&  40\% \\ \hline
% Sim 3 & \includegraphics[scale=0.1]{Figs/Teste_3-1_saida} 		& 30 agents & 7\% 	&  18\% 	& 16\% 	&  23\% \\ \hline
% Sim 4 & \includegraphics[scale=0.1]{Figs/Teste_4_salas} 		& 30 agents & -25\% &  -7\% 	& -21\% &  35\% \\ \hline
% Sim 5 & \includegraphics[scale=0.07]{Figs/Teste_5_corredor} 	& 20 agents & -3\% 	&   1\% 	& -2\% 	&  45\% \\ \hline
% Sim 6 & \includegraphics[scale=0.1]{Figs/4_small_rooms} 		& 28 agents & 36\% 	&  40\% 	& -15\%	&  18\% \\ \hline
% Sim 7 & \includegraphics[scale=0.1]{Figs/Teste_5_salas_funil} 	& 30 agents & -10\% &  -1\% 	& -25\% &  -7\% \\ \hline
% Sim 8 & \includegraphics[scale=0.1]{Figs/5_identical_rooms} 	& 20 agents & 26\% 	&  16\% 	& 14\% 	&  62\% \\ \hline
% Sim 9 & \includegraphics[scale=0.1]{Figs/7_identical_rooms} 	& 20 agents & 22\% 	&  13\% 	& 13\% 	&  54\% \\ \hline
% Sim 10 & \includegraphics[scale=0.1]{Figs/9_identical_rooms} 	& 20 agents & 20\% 	&  12\% 	& 13\% 	&  50\% \\ \hline
% \end{tabular}
% \quad
% \label{tab:env_err}
% \end{table*}

%After estimating each case, we obtained the data $\vec{ED_e}$ as described in Section~\ref{sec:env_estimator}. In addition, each environment was also modeled in 3D in Unity Engine and simulated generating $\vec{SD_e}$ to be used for comparison and evaluation with the estimated data. 
%We use the mean absolute relative error to measure the difference between the estimation and simulation for the tested environments. 
%Figure~\ref{fig:err_val} shows the measured error values for such 20 environments regarding total evacuation time $tt_e$ and average time $\bar{t}_e$ of environment $e$ when evaluated with simulations. In this figure it is easy to see that as the population distribution varies along the rooms (simulations $Sim1'$ to $Sim10'$ compared to results of simulations $Sim1$ to $Sim10$), the error value of average time $\bar{t}$ for each agent increases. It is expected in our method because each room is estimated only once for each full environment. It means that when the population is distributed in various rooms, people should wait for agents that should entry in a specific room in order to be estimated. For example, consider $Sim6'$ as illustrated in Table~\ref{tab:env_err}: if there are agents in the central room, those entities should wait for others that come from the other rooms in order to have the central room estimated by the ANNs. This characteristic impacts the parameters $\bar{t}$ of agents which are in this specific room.

Figure~\ref{fig:err_val} shows the measured error values for these 20 environments regarding total evacuation time $tt_e$ and average time $\bar{t}_e$ of environment $e$ when evaluated with simulations. In this figure it is easy to see that as the population distribution varies along the rooms (simulations $Sim1'$ to $Sim10'$ compared to results of simulations $Sim1$ to $Sim10$), the error value of average time $\bar{t}$ for each agent increases. It is expected in our method because each room is estimated only once for each full environment. It means that when the population is distributed in various rooms, people should wait for agents that should entry in a specific room in order to be estimated. For example, consider $Sim6'$: if there are agents in the central room, those entities should wait for others that come from the other rooms in order to have the central room estimated by the ANNs instead of leaving immediately. 
\blue{This characteristic impacts mainly the $\bar{t}$ of the environment since agents that would leave early need to wait for the late ones to start leaving, limiting the evacuation time of each agent by the time of the late ones. $tt$ should not be heavily affected simply because it is already based on the evacuation time of the last agents.}

Indeed, the obtained average errors for total evacuation time $tt$ for scenarios Sim1 to Sim10 is 20.9\%, while the average  error for scenarios Sim1' to Sim10' is 12.6\%. It can be interpreted that our method estimates reasonably well the total evacuation time for full environments, even if the population distribution varies, and we believe that this improvement observed is just a fluctuation of the results. However, our heuristic impacts the average time $\bar{t}$ parameter, as previously discussed. While the error of $\bar{t}$ for the first set of simulations is 14\%, the second set presented an error value of 35.9\%. In addition, the total evacuation time average error value for the 20 environments is 16.75\%.
%(from all 20 environments) when comparing estimation with simulation process; Average exit time got 31\% average error while the other two parameters got 65\% and 69\% average error , the standard deviations were 18\% and 26\% for Simulation time and Average exit time, and 32\% and 101\% for Average speed and Average density. These values can be seen in Figure~\ref{fig:env_avg}.

%The evaluation makes use of the absolute value of the difference between the predicted value and the real value divided by the real value to measure the size of the error of the estimation. In this case the result obtained in the simulation are the real values.



\subsection{Investigating Replicated Rooms}
\label{sec:Part2}

%Once the ANNs application in rooms can present an error, as it can our defined heuristic, in the estimation, this section aims to discuss that. 
We expect that the estimation will present errors if compared to full simulation. Errors can come from the ANNs error propagation, but still from our heuristics, as discussed in last section. In order to evaluate the error caused by our estimation, we chose 2 rooms from the 2000 ones used in validation. We selected the best and worst estimations presented in this set of environments. They are following named: $r_b$ and $r_w$, respectively for the best and worst estimated total evacuation times. %$r_b$ has following dimension $YY$ while XXXX. For the both rooms we simulated ZZ agents.
$r_b$ is a 28 meters wide 6 meters long room with 99 initial agents and a incoming flux 3.3 agents per second during 24.7 seconds with an exit 5.6 meters wide, while $r_w$ has 29.5x4.7 meters, 12 initial agents and 9.3 agents per second during 1.4 seconds and a 1.1 meters wide exit.
%Figure~\ref{fig:9rooms} illustrates one example of replicated rooms environment having 9 rooms.
%SO: Estevão como são essas duas salas? quantas pessoas tem?


%In addition, we used two specific rooms used in the validation phase. The first one was the room that presented the lower error in the room estimation, while the second one obtained the larger error. 
For each of those rooms, we generated new full environments by replicating the specific room structure (dimensions and exit size for $r_b$ or $r_w$) and connecting it to the original room. %Figure~\ref{fig:9rooms} illustrates one example of rooms replicated for the $r_b$ cases. 
\blue{By making cases in this way we assume that the error from the ANNs to estimate each room is constant, so it allows us to verify variations as a product of the heuristics.}

% \begin{figure}[htb]
% \centering
% \includegraphics[width=0.7\linewidth]{Figs/9_identical_rooms}
% \caption{Identical rooms placed in sequence in order to be estimated.}     
% \label{fig:9rooms}
% \end{figure}

This way we created 14 new cases for each room, each case with two more rooms than the last one. For instance, the first environment has only 3 rooms, then second environment has 5 rooms, then 7 rooms, 9 until 29 rooms. So, we generated new 28 environment cases, half of them replicating $r_b$ and half $r_w$. In all cases the agents are placed in the first room and must travel until the exit, i.e. the last room.
%In all cases the number of agents is fixed in 20 and all agents are placed in the first room in the hierarchy. %Our goal in this case was to observe the error generated through the propagation of ANNs method. 

For each one of the 28 new environments, in addition to the graph representation using our editor (see Section~\ref{sec:EnvEditor}), we also modeled the geometry using Unity. The goal is to simulate the environments in order to compare with the estimation results. To proceed with this analysis, we compared the estimation and simulation total evacuation time ($tt_i$) for each environment, as can be seen in Figure \ref{fig:propagErrors}. In the case of the best estimated room $r_b$ the average absolute relative error for all 14 environments is 18\% (Std.Dev=6\%)  while the average error for the 14 environments generated using $r_w$ is 29\% (Std.Dev=15\%). 
%
%Although these environments containing 29 rooms are very complex and maybe unrealistic, our maximum achieved errors is 30\%. 
We consider this as a good result since the error percentage did not increase as the number of rooms increased. It indicates that the propagation of the ANNs errors by our heuristics did not produce an ever growing error rate as the number of rooms increase, in fact it appears that it helps mitigates extreme cases into average cases. %Moreover, during the simulation the agents motion are organized, e.g. in lanes, what does not happen in estimations. % EST: a importância da organização em lanes foi explicada?

\begin{figure}[htb]
\centering
\includegraphics[width=1\linewidth]{Figs/propagErrors}
\caption{Absolute relative errors of the propagation cases.}
\label{fig:propagErrors}
\end{figure}

%Going further in this analysis, we decided to measure the error presented only with the ANNs estimation in the environment with 29 rooms, room-by-room, for $r_b$ and $r_w$. Comparing room by room the estimation and simulation we obtained for $r_b$ a average error value of 7.67\% (Std.Dev=12.75\%), while same analysis for $r_w$ resulted in 19.24\% (Std.Dev=6.42\%). It indicates that the error presented in the total evacuation time are impacted by the error generated by the ANNs estimation, but also by the defined heuristics. 
%SO: Aqui acima corrigir os valores.

%It is important to emphasize that such evaluations from simulated and estimated total evacuation time are not completely fair because during the simulation, the agents organize themselves in a corridor passing trough the doors. On the other hand, the estimation is executed room by room without considering any prior organization or data from the previous rooms. So, we proceed with a test where rooms could benefit from flow computed in previous rooms, just for cases where geometry rooms are the same as well as the number of people passing through the doors (exactly the example discussed in this section with replicated rooms). Results are as follows:
%SO: colocar dados aqui
 
 %SO: comentei abaixo. Acho que tem coisa estranha nestes dados :(
%Going further in this analysis, we decided to measure the error presented along the propagation of data during the estimation. We collected the local data of each room in the environment with 29 rooms through the simulation and estimation, for $r_b$ and $r_w$.

%Comparing room by room the estimation and simulation we obtained the following chart of relative errors between them, Figure \ref{fig:rbr}. In this chart it is visible that the error is being propagation forward during the estimation starting at 3\% and achieving 140\% relative error for $r_b$ propagation and from 50\% to 1100\% with $r_w$. This enormous growing of the relative error is expected as we are propagating the case with the greatest error found, however, comparing it with previous result we can notice final estimation heuristics manage to counter this ever growing error, fitting it into a much smaller error which appears to converge into a 15\% relative error.

% \begin{figure}[htb]
% \centering
% \includegraphics[width=1\linewidth]{Figs/roombyroom}
% \caption{Absolute relative error for total evacuation time ($tt_e$) of room-by-room estimations during the 29 rooms case estimation.}
% \label{fig:rbr}
% \end{figure}

\subsection{Testing a practical example}

In order to test our method in a practical example, we use the night club as described in~\cite{Cassol2017}. We used the same 3D environment as illustrated in Figure~\ref{fig:SM} to define the environment to be estimated using our editor and simulate it containing 940 agents.

\begin{figure}[htb]
\centering
\includegraphics[width=0.9\linewidth]{Figs/Nightclub}
\caption{Architecture of the nightclub used as base for simulation and estimation.}
\label{fig:SM}
\end{figure}

The 3D environment has 3 floors and many rooms. There are some rooms that have more than one exit (not yet dealt in our method), so we divided such rooms in two or more rooms each one, depending on the number of present exits. This decision makes possible to simulate the night club (and any other environment) using our work. Clearly, it can bring some errors. In a future work we want to address this feature. Figure~\ref{fig:SM2} shows the graph generated using our Editor to model the night club (named SM) in order to be estimated. 
%SO: arrumar as palavras que estão em portugues da figura ...
%EST: mais de uma saída até trata. O treinamento sempre foi com uma saida só, mas pra por os números pras salas com várias saídas dá sim. 

\begin{figure}[htb]
\centering
\includegraphics[width=0.9\linewidth]{Figs/SM}
\caption{Modeling of SM night club in our editor.} 
\label{fig:SM2}
\end{figure}
%SO: Estevao tens que mudar os nomes das rooms na fig...


For this practical result, we decided to measure the four metrics initially studied in this work (total evacuation time, average time, average speed and average density). The computed differences are presented in Figure~\ref{fig:SMerror}. As can be seen, the total evacuation time keeps an acceptable error around 30\%, as the average speed and density. On the other hand, the average exit time per agent presents a larger error mainly due to the fact that agents which are placed in each room wait for others who should entry in the specific room to be estimated. This issue was discussed in Figure~\ref{fig:err_val} and it will be the subject of a future investigation.
%SO: Estevao: para simplificar tira speed e density dessa fig...

\begin{figure}[htb]
\centering
\includegraphics[width=1.1\linewidth]{Figs/SMerror}
\caption{Errors in percentage as resulted from the comparison between the estimation and simulation of a practical example.} 
\label{fig:SMerror}
\end{figure}

In terms of required time to model and simulate environments as well as to estimate, follows a comparable analysis:
\begin{itemize}
\item \textbf{5-10 minutes} was the time to model the night club in our Editor, once the user has the floor plan with the detailed information needed of the environment; 
\item  \textbf{12-16 hours} is the time for a skillful designer to model the 3D environment, once s/he has the floor plan of the environment. Additionally, the time to prepare a 3D geometry to be simulated, using a crowd simulator is a complex task. The user has to learn how to operate a simulation software, define rooms to walk, place people and groups, define escape routes. The time to accomplish this task, using CrowdSim as defined in~\cite{Cassol2017}, to prepare the night club to be estimate can take \textbf{weeks}, and this is repeated for each new environment to be simulated.
\item  The environment estimation is instantaneous, i.e. to estimate the night club it takes \textbf{less than one second}.
\item As described in~\cite{Cassol2017}, a full simulation containing 240 agents in the night club executing at 24 frames/second takes around 3 minutes to evacuate the full environment.
\end{itemize}

Important to emphasize that, as discussed in~\cite{Cassol2017}, if we want to simulate various distribution of people in the night club, our method can also be used. We should easily define the amount of people in the rooms, e.g. scripting it or using our Editor, and instantaneously estimate the total evacuation time. In comparison with~\cite{Cassol2017} while using a granularity of 10 percent at the bifurcations (meaning this the difference among the exits), the plans with 240 agents took about 4 hours, and 1,010 agents took approximately 30 hours. It means that we could easily and quickly to find out the best evacuation plan for a specific population distribution, having an acceptable estimation error of 30\% in total evacuation time.

%We obtained errors for each of chosen metrics as follows: Simulation time obtained 17\% average error (from all 20 environments) when comparing estimation with simulation process; Average exit time got 31\% average error while the other two parameters got 65\% and 69\% average error , the standard deviations were 18\% and 26\% for Simulation time and Average exit time, and 32\% and 101\% for Average speed and Average density. These values can be seen in Figure~\ref{fig:env_avg}.


% \begin{figure}[htb]
% \centering
% \includegraphics[width=1\linewidth]{Figs/400-400-200-200_average.png}
% \caption{Obtained results when testing 20 environments. The average error size and standard deviation is shown for each estimated attribute.}     
% \label{fig:env_avg}
% \end{figure}

% \subsection{Training and validation\label{sec:trainingmodel}}

% For each attribute to be estimated (Simulation time, Average exit time, Average speed and Average density) it was trained a simple one hidden layer fully connected network with six hidden neurons and no bias. The loss function used was the mean squared error function. The training occurred intensively, only stopping when no more reduction on the loss was observed by new epochs even when altering the learning rate. With this network trained, the following individual validation errors was measured using the absolute of the difference between the predicted value and the real value. Here we measured the quality of our estimations according to how many cases were bellow 10\% error. The Simulation time network managed to have an astounding 89.5\% of the validation cases bellow 10\% error, the Average exit time network managed 72.3\% of the cases, meanwhile the Average speed and Average density networks 40.9\% and 45.7\% respectively. The errors histograms of these networks can be seen on figures \ref{fig:ST6neurons}, \ref{fig:AE6neurons}, \ref{fig:AS6neurons} and \ref{fig:AD6neurons}.

% \begin{figure}[htb]
% \centering
% \includegraphics[width=1\linewidth]{Figs/6Simulation_time__seconds_.png}
% \caption{Hidden layer with 6 neurons, simulation time error percentage.}     
% \label{fig:ST6neurons}
% \end{figure}

% \begin{figure}[htb]
% \centering
% \includegraphics[width=1\linewidth]{Figs/6Average_exit_time__seconds_.png}
% \caption{Hidden layer with 6 neurons, average exit time error percentage.}     
% \label{fig:AE6neurons}
% \end{figure}

% \begin{figure}[htb]
% \centering
% \includegraphics[width=1\linewidth]{Figs/6Average_speed__m_s_.png}
% \caption{Hidden layer with 6 neurons, average speed error percentage.}     
% \label{fig:AS6neurons}
% \end{figure}

% \begin{figure}[htb]
% \centering
% \includegraphics[width=1\linewidth]{Figs/6Average_density.png}
% \caption{Hidden layer with 6 neurons,average density error percentage.}     
% \label{fig:AD6neurons}
% \end{figure}

% Following the individual validation, these networks were validated working together to estimate the environments. The validations errors were measured using the absolute value of the difference between the predicted value and the real value are compared with the real value to measure the percentage error value. In the environment simulations the Simulation time got a whooping 22\% average error size while the other three parameters keep around 60\% average error, the standard deviations were significantly lower for each, 16\% and 15\% for Simulation time and Average exit time, and 10\% and 20\% for Average speed and Average density. These values can be seen on figure \ref{fig:6-6-6-6avg}.

% \begin{figure}[htb]
% \centering
% \includegraphics[width=1\linewidth]{Figs/6-6-6-6_average.png}
% \caption{Validation of estimated environments with 14 environment cases using networks with 6 hidden neurons. The average error and standard deviation of each attribute is shown.}     
% \label{fig:6-6-6-6avg}
% \end{figure}

% Despite our main objective being the creation of a methodology to allow the estimation of entire environments and not exactly the search for the best network to do so, we still searched for a better model. We did so by varying the quantity of neurons on the hidden layer and observing the individual results. New attempts were made using 50, 200, 400 and 500 neurons on the hidden layer. Each attempt efficiency was measured by collecting how many cases during individual validation were bellow 10\% error, they can be seen on figure \ref{fig:treinamentos}. The best configuration obtained for each attribute was with 400 neurons for the Simulation time and for Average exit time and 200 neurons for Average density. Average speed had nearly the same result with 200 and 400 neurons, 200 neurons was chosen because of its slightly smaller standard deviation during individual validation. With these new networks the number of cases bellow 10\% error improved for all attributes: from 89.5\% to 91.5\% in Simulation time, from 72.3\% to 85.4\% in Average exit time, from 40.9\% to 49.9\% in Average speed and from 45.7\% to 51.6\% in Average density. The error histograms can be seen on figures \ref{fig:ST400neurons}, \ref{fig:AE400neurons}, \ref{fig:AS200neurons}, \ref{fig:AD200neurons}.

% \begin{figure}[htb]
% \centering
% \includegraphics[width=1\linewidth]{Figs/scattertraining.png}
% \caption{Search for a better network model. Attempts with 6, 50, 200, 400 and 500. Plotted number of cases bellow 10\% error in the individual validation.}     
% \label{fig:treinamentos}
% \end{figure}

% \begin{figure}[htb]
% \centering
% \includegraphics[width=1\linewidth]{Figs/400_neurons_-Simulation_time__seconds_.png}
% \caption{Hidden layer with 400 neurons, simulation time error percentage.}     
% \label{fig:ST400neurons}
% \end{figure}

% \begin{figure}[htb]
% \centering
% \includegraphics[width=1\linewidth]{Figs/400_neurons_-Average_exit_time__seconds_.png}
% \caption{Hidden layer with 400 neurons, average exit time error percentage.}     
% \label{fig:AE400neurons}
% \end{figure}

% \begin{figure}[htb]
% \centering
% \includegraphics[width=1\linewidth]{Figs/200_neurons_-Average_speed__m_s_.png}
% \caption{Hidden layer with 200 neurons, average speed error percentage.}     
% \label{fig:AS200neurons}
% \end{figure}

% \begin{figure}[htb]
% \centering
% \includegraphics[width=1\linewidth]{Figs/200_neurons_-Average_density.png}
% \caption{Hidden layer with 200 neurons,average density error percentage.}     
% \label{fig:AD200neurons}
% \end{figure}



% Validating these new networks with the environments cases, figure \ref{fig:400-400-200-200}, improvements in the Simulation time, Average speed and Average density can be observed, from 22\% average error to 19\%, 61\% to 52\% and 53\% to 46\% respectively, while maintaining basically the same standard deviation. Average exit time remained with 30\% average error, however its standard deviation got a slight improvement of 3\%.

% \begin{figure}[htb]
% \centering
% \includegraphics[width=1\linewidth]{Figs/400-400-200-200_average.png}
% \caption{Validation of estimated environments with 14 environment cases using networks with 400 hidden neurons for Simulation time and Average exit time and 200 neurons for Average speed and Average density. The average error and standard deviation of each attribute is shown.}     
% \label{fig:400-400-200-200}
% \end{figure}

%AQUI propagation
%\subsection{Propagation model validation}

% One concern this use of data being propagated between rooms may raise is the possibility of propagating the errors from the estimations forward during the environment estimation. These errors may accumulate along the estimation process, bringing the result for each iteration of the propagation further away from the real value.

% To investigate how this problem affects the model we isolated the two validation rooms that had the best and the worst estimation for the Simulation Time. Then we proceed by creating cases to test the propagation of such rooms, each case is a series of rooms identical to the ones in the validation. Agents are spawned in the first room of the series as they were in the validation room, however the exit is positioned at the end of the series. This way we generated 15 environments for each isolated room, increasing the number of rooms by two in each case, varying the number of rooms from 1 to 29.

% The comparison between the estimated an the simulated results can be seen on Figure \ref{fig:propag} for the propagation of the room with the worst estimation of the Simulation Time and Figure \ref{fig:propagmenor} for the room with the best estimation. 

% \begin{figure}[htb]
% \centering
% \includegraphics[width=1\linewidth]{Figs/propag.png}
% \caption{Estimation of 15 environment cases for investigating the propagation behavior. Each case is composed of a consecutive series of rooms, varying from 1 to 29 rooms. Each color is the result of a different case ordered by the number of rooms, from the fewest (black) to the most (red). }     
% \label{fig:propag}
% \end{figure}

% \begin{figure}[htb]
% \centering
% \includegraphics[width=1\linewidth]{Figs/propagmenor.png}
% \caption{Estimation of 15 environment cases for investigating the propagation behavior. Each case is composed of a consecutive series of rooms, varying from 1 to 29 rooms. Each color is the result of a different case ordered by the number of rooms, from the fewest (black) to the most (red). }     
% \label{fig:propagmenor}
% \end{figure}

%Observing the results obtained on this evaluation, we detect that the error size converges as the number of rooms present increases. This convergence indicates that the error propagation has a limitation on this model.

==> 5_remarks.tex <==
In this document we proposed a methodology for estimating evacuation data for complex  environments, instead of simulating it. We used ANNs to train and estimate data for separated rooms individually, considering their geometry and population. Then, using such estimations, we propose an heuristic to estimate full environment parameters as total evacuation time and average time per agent.% to estimate the data for the entire environment. We have elaborated all steps of its development, from the creation of a crowd simulator to generate databases of simulations used for training and validation, to the training of neural networks for estimating data of rooms, and how to merge all this data together in a complete environment estimation.

The approach we used to train ANNs with separated rooms and then aggregate data using a simple heuristic seems promising. We achieve less than 20\% of error when comparing estimation and simulation results for 2000 rooms and approximately 50 full environments, where complexity was reasonable, e.g. environments with 29 rooms. The other alternative was to train the ANNs with several full environments instead of separating them in rooms. Further investigations on this approach is one of our next projects for future.%Specifically, in this paper we investigated environments composed by rectangular rooms that have only one exit. 

Analyzing the obtained results we can see that there is still room for improvements. The neural network estimations can be further explored, by using deeper network models and by increasing the database (currently we have 18000 rooms in the training database). These improvements can reduce the error size of the results obtained, specially for the Average speed and Average density since they are the ones with lower accuracy in our method to estimate rooms.

%Analyzing the results obtained we can clearly see that there is still room for improvements. The neural networks estimation is nothing near perfection, especially for the Average speed and Average density attributes. Despite that, by comparing the result obtained, we can observe that the evolution of the environment validation accompanied the evolution on individual validation, which is a sign that by searching and improving the neural networks we can keep on improving the estimations on the environment. This is true for all attributes but the Average exit time. It having the the worst result on the environment validation while having one of the greatest individual results (second, losing only to the Simulated time) can only be a sign that the metric to merge the rooms estimations into the environment estimation needs improvements.

%The fact that the estimated error size converge as the number of rooms increases indicates that the methodology does not propagate the errors forward, in fact it may even correct possible bad estimations along the propagation.

\blue{With respect to the limitations of the model: the training database was created solely with abstracted rooms, containing only one entrance and one exit directly opposed to the entrance, which may not always be the case in the environments to be tested. One way to improve the versatility of the model and to approach its usability for real cases is to add more parameters which are important to define the rooms, like multiple doors and exits. Obstacles are an entire issue themselves, since there is a lot of information about them: shape, size, position, orientation, etc, for each obstacle present. In order to not loose too much the abstraction of the model, we suggest creating a "level of obstruction" parameter for the rooms, with a value of 0 meaning the room is free of obstacles and can be transversed without problems and increasing as the obstacles impairs the movement of the agents. Defining this parameter would greatly improve the similarity of the model with reality and we think it is worth a research of its own.}


Observing the tested environments, we detect another limitation imposed by our approach to combine ANNs and the post-processing heuristic. It happens specifically for rooms which have dependence rooms and also have an initial population on it. Indeed, since the estimation (using ANNs) of these rooms could only be executed when all dependence rooms have finished their estimation, it generates a conceptual issue once people, in this type of room, only start to move when people from dependence rooms arrive. We measured this issue in the tests presented in Figure~\ref{fig:err_val} and as could be seen, this characteristic of our method impacts clearly the average time per agent (what is expected, since one agent in a specific room should wait for people who entry in this room in order to start to move). On the positive side it did not impact the total evacuation time. We intend to improve our heuristic in this issue.

Finally, the tests performed in a practical example (using one tested environment in real life) was very promising. 
\blue{The estimation error of total evacuation time was less than 30\%. Although this number may appear high, it is the result of a comparison with crowd simulations, which already has a distance from reality, and even real evacuation drills lack accuracy when comparing with real evacuation scenarios, table \ref{tab:nightclubtimes} shows the Evacuation time of the night club provided by Cassol et al. \cite{Cassol2017} and the one we obtained in the simulation and estimation we realized in this same scenario. In addition, we imagine that this accuracy nicely compensates the facts that the user do not need to model the 3D environment, learn how to use and prepare the simulation in a crowd simulator, test simulations and finally wait hours for results.}

\begin{table}[h]
\centering
\begin{tabular}{|p{1.25cm}|c|c|c|c|}
\hline
 & \multicolumn{2}{|c|}{\centering Cassol et al. \cite{Cassol2017}}
 & \multicolumn{2}{|c|}{\centering Our work} \\ \hline
 & Real drill & Crowdsim  & Simulation & Estimation \\ \hline
 Evacuation time & 175s & 142s & 230s & 294s \\ \hline
 Relative error & | & -18\% & | & +28\% \\ \hline
\end{tabular}

\quad

\caption{Nightclub evacuation time from different sources.}
\label{tab:nightclubtimes}
\end{table}

As described in results, this task can save weeks (maybe months) of work. We believe our tool is a further step in the direction to have all environments from real life simulated and tested, once this tool can clearly facilitate the work.

%we remember that the main objective of this work was to propose the estimation model and validate if it is able to predict the evacuation data, more search for better parameters, neural network models and heuristics are something for future works, . Besides

% \begin{figure}[htb]
% \centering
% \includegraphics[width=1\linewidth]{Figs/400-400-200-200.png}
% \caption{Individual estimation of the 20 environment cases for validation. Second half of the cases have a identical structure of the first half, but the agents are distributed evenly among the rooms. }   
% \label{fig:environments}
% \end{figure}

%for the rooms with found is that during the environment estimation each room with dependencies waits for its dependencies to be estimated before being estimated. In the case of a room with dependencies and with a initial population it may be interpreted as that the people of this room waits for the people on the other room to catch up with them to start evacuating. 
%For this reason, the tested case which presented the smaller relative error in comparison to the simulations is the one where initial positions of agents are into the rooms without dependencies i.e. the farthest rooms from the exit in the environment, as can be seen in Figure \ref{fig:environments}.% (Ref figura e mostrar se é verdade que onde tinha mais gente "no caminho" era o caso com mais erro...)(FALTAM DADOS AQUI)
%SO: estevao, esses dados não existem no paper.. a gente simplesmente nao tem os dados por case. só as medias...
%SO2: Aqui continua ruim :( não dá apra ver que acertamos mais quando tinham agents só na primeira sala...

%When talking about emergency simulations, and the impact this kind of technology can have in people's life, we believe it is preferable to be wrong by increasing the needed time to evacuate, then doing the opposite. So, if our heuristic lacks of realism while waiting for dependence rooms to estimate the global time, our method is very adequate to simulate the worst case scenarios.
%SO2: Aqui está ruim também ... não mostramos que erramos só para cima...
%AQUI poderiamos colocar explicitamente estes valores e simular os ambientes (os 13?) sempre com pessoas na primeira sala e avaliar o erro... para ver se isso é vverdade...

%On the positive side, we do believe that this characteristic of our model allows us to simulate the worst case scenario, i.e. people in the environment are located in the rooms which are faraway from the exits. 
%In a future work, we want to improve our database to train and test rooms with different configurations, e.g. number of exits and their distribution in the room geometry. In addition, we want to improve our global heuristic to the environment to propose a local way to consider the populations and dependences for each room.
%An evacuation with the agents located in the farthest points can be interpreted as a worst case scenario to be evacuation, which is the most crucial evacuation to be made, but still is a limitation of the model.

\section*{Acknowledgment}

The authors would like to thank Brazilian agencies (CNPq and CAPES) and ONRG for supporting our research.

==> Makefile <==
# make -f Makefile_latex

R = template
STY = *.cls
FIG = images/samplefigure.pdf

pdf: $(R).pdf

$(R).bbl: $(R).bib
	latex $(R)
	bibtex $(R)
	latex $(R)

$(R).ps: *.tex $(STY) $(FIG) $(R).bbl
	latex $(R)
	dvips -Ppdf -G0 -t letter $(R)

$(R).pdf: $(R).ps
	ps2pdf -dPDFSETTINGS=/prepress \
	-dCompatibilityLevel=1.4 \
	-dAutoFilterColorImages=false \
	-dAutoFilterGrayImages=false \
	-dColorImageFilter=/FlateEncode \
	-dGrayImageFilter=/FlateEncode \
	-dMonoImageFilter=/FlateEncode \
	-dDownsampleColorImages=false \
	-dDownsampleGrayImages=false $(R).ps $(R).pdf

clean:
	rm -f $(R).log $(R).aux $(R).bbl $(R).blg $(R).dvi $(R).ps $(R).out

